(S)GD over Diagonal Linear Networks: Implicit Regularisation, Large Stepsizes and Edge of Stability

In this paper, we investigate the impact of stochasticity and large stepsizes on the implicit regularisation of gradient descent (GD) and stochastic gradient descent (SGD) over diagonal linear networks. We prove the convergence of GD and SGD with macroscopic stepsizes in an overparametrised regression setting and characterise their solutions through an implicit regularisation problem. Our crisp characterisation leads to qualitative insights about the impact of stochasticity and stepsizes on the recovered solution. Specifically, we show that large stepsizes consistently benefit SGD for sparse regression problems, while they can hinder the recovery of sparse solutions for GD. These effects are magnified for stepsizes in a tight window just below the divergence threshold, in the "edge of stability" regime. Our findings are supported by experimental results.

==> Sections/shape_old.tex <==
\subsection{The shape of $\rm Gain _\gamma$ explains the differences between GD and SGD}
In this section,
% for simplicity 
we restrict our analysis to single batch SGD ($b=1$) and full batch GD ($b=n$).
%, \textit{i.e.,} $b = 1$ and $b = n$, respectively. 
While up to now our results do not involve any assumption on the data, we here focus for the sake of clarity on tractable noiseless sparse recovery setting (\cref{ass:sparse_reg_setup}), wherein the minimum $\ell_1$-norm interpolator is also the sparsest interpolator \cite{candestao}. 
The first part of \cref{ass:RIP1} closely resembles the classical restricted isometry property (RIP) and is relevant for GD while the second part is relevant for SGD. Such an assumption is not restrictive and holds with high probability for Gaussian inputs $\mathcal{N}(0, \sigma^2 I _d)$ (see \cref{lem:concentration_ripsgd} in Appendix). We study separately uncentered data in Appendix~\ref{app:uncentered}.
The precise assumptions are stated below. 
\begin{assumption}\label{ass:sparse_reg_setup}
There exists an $s$-sparse ground truth vector $\beta^\star_{\rm sparse}$ where $s$ verifies $n=\Omega(s\ln(d))$, such that $y_i=\langle\beta^\star_{\rm sparse}, x_i\rangle$ for all $i\in[n]$.
\end{assumption}
\begin{assumption}\label{ass:RIP1}
There exists $\delta, c_1, c_2 > 0 $ such that for all $s$-sparse vectors $\beta$, there exists $\varepsilon \in \R^d$ such that $(X^\top X) \beta = \beta + \varepsilon$  where $\Vert \varepsilon \Vert_\infty \leq \delta \Vert \beta \Vert_2$ and 
$ c_1 \Vert \beta \Vert_2^2  \mathbf{1} \leq \frac{1}{n} \sum_i  x_i^2 \langle x_i, \beta \rangle^2 \leq c_2 \Vert \beta \Vert_2^2 \mathbf{1}$.
\end{assumption}

We first  visualise in \Cref{fig:Gain} (right) a typical shape of $\rm Gain _\gamma$ from SGD and GD  trained with large stepsizes.
%near the edge of stability, where we see the most dramatic  difference between SGD and GD in \Cref{fig:main_theorem}. %\sg{chk: vs alpha-inf}  
In \Cref{fig:Gain} (right), we see that GD and SGD indeed lead to different shapes of $\rm Gain _\gamma$. 
Importantly, we see that for GD,  the  magnitude of $\rm Gain _\gamma$ is higher for coordinates in the support of $\beta^\star_{\ell_1}$. 
This is undesirable as based on our discussion above: the coordinates with high gain magnitude are adversely weighted in the asymptotic limit of $\psi_{\balpha_\infty}$. This would explain the observation that GD in this regime has bad sparse recovery guarantees in spite of having small scale of $\balpha_\infty$. 




\begin{figure}[t]
\centering
\begin{minipage}[c]{.5\linewidth}
\hspace*{-15pt}
\includegraphics[width=0.99\linewidth]{Figures/centered_scale2.pdf}
\end{minipage}
\hspace*{-15pt}
\begin{minipage}[c]{.5\linewidth}
\includegraphics[width=0.99\linewidth]{Figures/centered_EOS_GD_SGD.pdf}
% \caption{SGD $b=1$\label{subfig:sgd}}
\end{minipage}
\hspace*{-15pt}
\caption{ \textit{Left:} the scale of $\rm Gain_\gamma$ explodes as $\gamma \to \tilde{\gamma}_{\rm max}$ for both GD and SGD. \mathieu{def $\tilde \gamma$}
\textit{Right:} The shape of $\rm Gain_\gamma^{\rm SGD}$ is homogeneous whereas that of GD is heterogeneous with much higher magnitude on the support of $\beta^\star_{\ell_1}$ (first two coordinates on the left of the dashed vertical line). The shape of $\rm Gain_{\gamma}^{\rm GD}$ matches that of the gradient at initialisation.\label{fig:Gain}}
\end{figure}


The \textbf{shape} of $\rm Gain _\gamma$ is determined by the sum of the squared gradients $\sum_k \nabla \cL_{\cB_k}(\beta_k)^2$, and in particular by the degree of heterogeneity among the coordinates of this sum.
Precisely analysing the sum over the whole trajectory of the iterates $(\beta_k)_k$ is technically out of reach. However, we empirically observe for the trajectories shown in \Cref{fig:Gain} that the shape is largely determined within the first few iterates and that the shape of the whole sum is close to that $\mathbb{E}[ \nabla \cL_{\cB_k}(\beta_0)]$, motivating the following assumption.
\Snote{all this is messy, idk what's the best way of writing all this}

\begin{assumption}
    \label{ass:shady} There exists $\eta, c_3 > 0$ such that
     $\sum_k \nabla \cL_{\cB_k}(\beta_k)^2 \in c_3 [1-\eta, 1+ \eta] \mathbb{E}[ \nabla \cL_{\cB_0}(\beta_0)^2] $, where the expectation is taken w.r.t.~$\cB_0$.
\end{assumption}


The following proposition then shows that while the sum stochastic gradients squared of SGD are homogeneous, it is not the case for that of the gradients squared of GD. 
As a consequence, when the amplitude of the gain increases (which is the case when we increase the stepsize, as explained in the previous section), \textbf{the recovery of sparse vector in hindered for GD} (the coordinates to recover become heavily penalised), while \textbf{SGD favors sparse solutions}.


\begin{proposition}%[Shape of the (stochastic) gradient at initialistion]
\label{lemma:shape_SG_init}
Under \Cref{ass:sparse_reg_setup,ass:RIP1,ass:shady}, the sum of the (stochastic) gradient squared along the trajectory satisfies:
% \begin{align}
%     \nabla \cL &(\beta_0  )^2 = (\beta^\star_{\rm sparse})^2  + \varepsilon \,, \label{eq:nabla0_GD} \\
%     \mathbb{E}_{i_0} [\nabla &\cL_{i_0}(\beta_0)^2] = \Theta \Big(  \Vert \beta^\star \Vert_2^2 \mathbf{1} \Big)\,. \label{eq:nabla0_SGD}
% \end{align}
%
% \begin{align}
%     \frac{1}{C }\big((\beta^\star_{\rm sparse})^2  + \varepsilon\big)\leq \sum_{k<\infty} \cL(\beta_k)^2 \leq C\big((\beta^\star_{\rm sparse})^2  + \varepsilon\big)\quad \text{for GD}\,,\label{eq:nabla0_GD} \\
%     \frac{1}{C}\Vert \beta^\star \Vert_2^2 \mathbf{1}\leq \mathbb{E}_{i_k} [\nabla \cL_{i_k}(\beta_k)^2] \leq C \Vert \beta^\star \Vert_2^2 \mathbf{1} \quad \quad \text{for SGD}\,. \label{eq:nabla0_SGD}
% \end{align}
\begin{enumerate}
    \item $\sum_{k<\infty} \cL(\beta_k)^2 = \Theta\left( (\beta^\star)^2 + \varepsilon \right)$ for \textbf{GD}. 
    Since $\beta^\star_{\rm sparse}$ is sparse by definition, we deduce that the sum of the squared gradients along the trajectory is heterogeneous and that it takes larger values on the support of $\beta^\star_{\rm sparse}$: $\rm Gain _\gamma$ \textbf{has much larger values on the support of~$\beta^\star_{\rm sparse}$}, and the corresponding weighted $\ell_1$-norm therefore has bigger weights penalising the coordinates which belong to the support of $\beta^\star_{\rm sparse}$, which is harmful for the recovery of $\beta^\star_{\rm sparse}$ (as explained in Example~\ref{app:example}, Appendix~\ref{sec:app:example}).
    \item $\mathbb{E}_{i_k} [\nabla \cL_{i_k}(\beta_k)^2]=\Theta\left(\Vert \beta^\star \Vert_2^2 \mathbf{1}\right)$ for \textbf{SGD}.
    Hence, the gain vector $\Gain_\gamma$ for SGD is homogeneous and the corresponding weighted $\ell_1$-norm is therefore close to the uniform $\ell_1$-norm and the classical $\ell_1$ recovery guarantees are expected.
\end{enumerate}
%\textbf{(i)} $\sum_{k<\infty} \cL(\beta_k)^2 = \Theta\left( (\beta^\star)^2 + \varepsilon \right)$ for GD; \textbf{(ii)} $\mathbb{E}_{i_k} [\nabla \cL_{i_k}(\beta_k)^2]=\Theta\left(\Vert \beta^\star \Vert_2^2 \mathbf{1}\right)$ for SGD.


\end{proposition}


% \myparagraph{$\Gain_\gamma$ for GD is heterogeneous.}  Since $\beta^\star_{\rm sparse}$ is sparse by definition, from \textbf{(i)} (\cref{lemma:shape_SG_init}) we deduce that the sum of the squared gradients along the trajectory is heterogeneous and that it takes larger values on the support of $\beta^\star_{\rm sparse}$. Hence, $\rm Gain _\gamma$ \textbf{has much larger values on the support of $\beta^\star_{\rm sparse}$}. The corresponding weighted $\ell_1$-norm therefore has bigger weights penalising the coordinates which belong to the support of $\beta^\star_{\rm sparse}$, which is harmful for the recovery of $\beta^\star_{\rm sparse}$ (as explained in Example~\ref{app:example}, Appendix~\ref{sec:app:example}).

% \myparagraph{$\Gain_\gamma$ for SGD is homogeneous.}  On the contrary, from \textbf{(ii)} (\cref{lemma:shape_SG_init}), we have that the gain vector $\Gain_\gamma$ for SGD is homogeneous.
% The corresponding weighted $\ell_1$-norm is therefore close to the uniform $\ell_1$-norm and the classical $\ell_1$ recovery guarantees are expected.

In this section, we interpreted the implicit bias formulated in \cref{thm:implicit_bias} by studying the scale and shape of the gain vector $\Gain_\gamma$, and showed that large stepsizes consistently benefit SGD for sparse regression problems (uniform and large $\Gain_\gamma$), while the recovery of sparse vectors is hindered with large stepsizes for GD, for which $\Gain_\gamma$ becomes heterogeneous, with spikes on the coordinates to recover. In next section, we relate heurstically these findings to the \emph{Edge of Stability} phenomenon.

